Active and Passive Causal Inference Learning

This paper serves as a starting point for machine learning researchers, engineers and students who are interested in but not yet familiar with causal inference. We start by laying out an important set of assumptions that are collectively needed for causal identification, such as exchangeability, positivity, consistency and the absence of interference. From these assumptions, we build out a set of important causal inference techniques, which we do so by categorizing them into two buckets; active and passive approaches. We describe and discuss randomized controlled trials and bandit-based approaches from the active category. We then describe classical approaches, such as matching and inverse probability weighting, in the passive category, followed by more recent deep learning based algorithms. By finishing the paper with some of the missing aspects of causal inference from this paper, such as collider biases, we expect this paper to provide readers with a diverse set of starting points for further reading and research in causal inference and discovery.

==> hybrid_ci.tex <==
\section{ Active+Passive (Hybrid) CI Learning}


==> intro_old.tex <==
\section{Introduction}

{\em Do you believe in the principle that everything has a cause?} There can be challenges and oppositions to such a question. Suppose the statement is true, then what is the origin of the first cause and how did this first cause manifest itself? Another example of criticism would be how do we determine the cause when there are infinitely many possible causes in our universe? Unfortunately, we would not be able to prove such a kind of statement either. And yet, our instinct has the strong will to say “yes!” to this question. 
The human desire for comprehensive cognition is often satisfied by the comprehension of causal relationships and their effects. This tendency to seek causality may stem from the innate inclination to attribute causality to phenomena and to strive for a complete understanding of the world.

The human curiosity and the desire to understand how things work lead to studying causality \citep{Celeste2015, Zheng2020HowCI, ferraro2019, Bender2020}. Causality is to discover the causal relationship between variables. Causality delineates an asymmetric relationship where it can only say {\em “A causes B”} or {\em “B causes A”}, while the correlation expresses a symmetric relationship that measures the occurrence of A and B. Being able to depict the causal relationship is an ideal framework for humans to explain how the system works. 


In conjunction, humans are prediction living systems where we constantly predict and simulate future outcomes based on our past experience on both short and long-term scales. Such a characteristic makes us not only satisfied with discovering the causal relationship but also strive towards optimizing our decisions by estimating causal effect \citep{rubin2005causal, Nichols2007, Pearl09a, ahmed_2014, Hagmayer2017, Zheng2020HowCI, Loría2021}. The causal effect is realizing potential outcomes that are consequences of a choice of actions. For example, what are the outcomes of taking versus not taking a Covid-19 vaccine? In order to know the effect of Covid-19 vaccination, it requires predicting the outcome of both taking and not taking the vaccine. In general, the process of inferring the potential outcome given an action is called causal inference (CI). 

%Understanding the causal relationship and causal effect together may fulfill a human’s impulse toward better cognition. We wonder if this provokes us to hope that everything has a cause and ultimately we can understand them. Statistical causality and CI modelling can come in handy as a tool to assist us with understanding causal relationships and causal effects. While human predictions and intuitions are not quantifiable, the statistical models give us quantifiable output which provides us with better information.

%Indeed working with statistical models comes with data generation process assumptions. Mapping out the causal relationship from the entire system is impractical. Often, in statistical modelling, one narrows down the scope by reducing the number of variables and applying causality methods \cite{Lagnado2002, Pearl09a, Pearl2009, Grotzer2012, Shanmugam2015, Zhang2017, Heinze2018, Schölkopf2021, Guo2021}. This can be viewed as a top-down approach where we find a causal graph and then proceed with causal inference. Alternatively, we can simplify the causal graph by applying domain knowledge from the experts, and shifting the focus toward understanding the causal effect. This is a bottom-up approach and has immediate practical relevance to various applications. In this literature review paper, we study CI methods given a causal graph as means of finding ways to apply causal effects in practice. 

Statistical causality and CI modelling can be leveraged as tools to facilitate our comprehension of causal relationships and effects. While human predictions and intuitions are not easily quantifiable, statistical models can provide quantifiable outputs that furnish us with more precise and accurate information.
The use of statistical models is contingent upon certain assumptions regarding the data generation process. Due to the complexity of the entire system, it is often impractical to fully map out the causal relationships between variables. As such, statistical modelling typically involves narrowing the scope by reducing the number of variables~\cite{Lagnado2002, Pearl09a, Pearl2009, Grotzer2012, Shanmugam2015, Zhang2017, Heinze2018, Schölkopf2021, Guo2021}. This approach can be considered a top-down approach in which a causal graph is first identified, followed by causal inference. Alternatively, one may simplify the causal graph by applying domain knowledge from experts and focusing on understanding the causal effect. This approach can be viewed as a bottom-up approach, which is highly relevant to practical applications. In this review paper, we examine various methods of causal inference given a causal graph, with the aim of finding ways to apply causal effects in practical scenarios.

Despite the perception that CI is more practically manageable than causality, it is associated with its own theoretical and practical challenges. The most salient of these challenges is the fundamental problem of CI \cite{Pearl09a, Pearl2010}. This problem arises from the fact that we can only observe the outcome of a single action given a particular state, and not the outcomes of all possible actions. For example, in the case of medical treatment, we can either administer a vaccine or withhold it and observe the outcome, but we cannot observe both outcomes simultaneously. Consequently, it is impossible to determine whether a counterfactual action is superior or inferior to the chosen action, or whether a potential outcome prediction based on a counterfactual action is accurate or inaccurate. The former and latter challenges correspond to model estimation and evaluation problems, respectively, rendering the practical application of CI uncertain in real-life situations \cite{Kuroki2014, Pearl2021}.

%While CI has the perception of being more practically manageable than causality, it has its own theoretical and practical challenges. The most obvious one is the fundamental problem of CI \cite{Pearl09a, Pearl2010}. That is we can never observe the outcomes of all actions given a state, but only observe one action. For example, we can only vaccinate or not vaccinate a patient and observe the result of a patient, but not both. Thus, it is impossible to check 1) whether a counterfactual action is better or worse than the chosen action, and 2) whether a potential outcome prediction given a counterfactual action is correct or wrong. The former and latter correspond to model estimation and evaluation problems respectively, and they make it dubious to apply in real-life applications \cite{Kuroki2014, Pearl2021}. 

{\em Is it worth studying CI even after the fundamental problem of CI?} The counter to this question is that it is not just our statistical models but humans face the same problem as well. However, humans are arguably good at inferring causal effects depending on the problems\footnote{We are not claiming that humans can do a perfect causal effect but its approximation based on their mental statistical association tends to be good for some cases.} \cite{Penn2007, Hayley2019, Tolmie2022}. For example, in order to go from one place to another place, it is common to compare which route is faster. We have some good ideas of key confounders such as time and road conditions from our past experiences and are able to predict the effects of our choices. In contrast, we are not good at predicting whether a new drug will cure an illness compared to existing drugs. The former is an interpolation-based prediction from our past experience, whereas the latter is more of an extrapolation-based prediction. The former example is a good enough reason for us to study how we can successfully learn a CI model for interpolation problems.

Although humans do CI every day, we use on feelings and intuitions to make predictions and judgements. Therefore, we often tend to confuse ourselves from correlation results to causation \cite{Harnad2000, Matute2015, Blanco2018}. Correlation does not imply causation, at the same time, it is possible to have causation with no correlation. CI is tricky like that, because the conditional probability is not the same as the intervention probability, which we explain in the next section. Taking a statistical approach allows us to distinguish between correlation and causation by clearly defining the two probabilities.

Inferring causal effect requires measuring intervention probabilities. Intervention probability is the probability of outcome when we intervene in the system which is different from conditioning.  Unfortunately, we have access to conditional and joint probabilities, but not intervention probabilities. The ways to measure intervention probability using conditional probabilities have always been a huge research topic in many disciplines \cite{rubin1974estimating, berry1985bandit, Heckman1997, Weitzen2004, Hernan2006, Breslow2009, Graepel2010, Banerjee2012, Yazdani2015, Bouneffouf2020} and there exists enormous work on various assumptions and conditions that allows us to infer causal effects \cite{rubin1974estimating}. The most basic assumptions are i) exchangeability, ii) positivity, iii) consistency, and iv) no interference. In the next section, we thoroughly review each assumption and its implications.

The burden of satisfying assumptions and conditions is subject to the data collection process rather than modelling. This is because the statistical models that we work on estimate statistical quantities, and not causal quantities. These are assumptions that enable us to convert causal quantities to statistical quantities, and they should be applied to causal graphs from which data are generated  \cite{Miguel2019, Rashelle2019, Zheng2019}.  One obvious way to achieve this is by randomly allocating data among all actions. Often a random controlled trial (RCT) is used in scientific experiments and clinical trials, where patients are given random treatment or control assignments \cite{Chalmers1981, Kendall12003, Aronow2021}. RCT is deliberately designed to be unconfounded between the treatment and the confounder which makes the study unbiased. This unbiasedness implies that the conditional probabilities from RCT data approximate the intervention probabilities. 

Nevertheless, randomized data collection is not always available and often suffers in efficiency from running large-scale experiments. There has been enormous work from various disciplines on estimating causal effects without fully randomized datasets \cite{rubin1977assignment, Rubin1979UsingMM, Chalmers1981, Lu2004OptimalPM}. As an alternative to randomized data, existing methods includes either to figure out how to work with the non-randomized dataset or find a way to intervene in the data collection system. In this paper, we organize CI methods into passive and active learning approaches. Passive CI learning refers to methodologies that work with given datasets, which were passively collected by the experts. In contrast, active CI learning refers to methodologies where we have options to actively intervene in the data collection process. RCT is an active way of collecting data by randomizing the treatment assignment. In other active CI learning method, we can have a trade-off between exploration and exploitation.  

The organization of this literature review paper is as follows. In section 2, we introduce the definitions and metrics for estimating causal effects, and assumptions used for identification. We also cover naive conditional mean estimator and ordinary square estimator that are widely applied to randomized datasets \cite{rubin1974estimating, Pearl2010}. 


In section 3, we describe RCT and then dive into bandit approaches to tackle active CI methods. While bandits are used in many practical applications, the research community has been adding more emphasis on theoretical analysis of minimizing the regret bounds of different policy algorithms \cite{berry1985bandit, Langford2007}. We look at bandits through the lens of CI where many of the bandit algorithms can be seen as learning the classic causal graph in Figure~\ref{fig:ci_causal_graph} with different exploration and exploitation rates. We examine different constrained contextual bandit problems by considering different causal graph scenarios. We also compare passive CI learning methods to bandits on naive causal graphs. Additionally, we review causal bandits which consider a graph with unknown confounding variables \cite{Bareinboim2015, Lattimore2016, Sachidananda2017OnlineLF}. In this survey, we do not cover causal reinforcement learning as it involves more reward and credit assignments over interdependent action and state variables, and requires relaxing some of the assumptions.

In section 4, we discuss the fundamental passive CI methods, which include matching \cite{RUBIN1992, Gu1993ComparisonOM}, inverse probability weighting \cite{ROSENBAUM1983, RUBIN1992, Hirano2003}, double robustness methods \cite{Bang2005, Shardell2014, Seaman2018}, and deep learning based CI methods\cite{Cai2012, Pearl2015, Johansson2016, Wang2016}. The recent deep learning literature has focused on learning representation while performing causal inferences \cite{Louizos2017}. Often deep neural networks are applied to high dimensional data with very complicated mapping from input to output. One of the big advantages of using deep learning approaches is to learn a representation that captures the intrinsic and semantic intermediate representations of data \cite{Kingma2014, Rezende2014}. Deep learning is applied to CI in order to infer causal effects by learning the hidden/unknown confounder representations from complicated data and causal graph relationships. For example, this type of method can work with raw medical images, treatments, unknown confounders in the image, and the relationship between the confounders to the outcomes \cite{Castro2020, Im2021, Puli2022, Amsterdam2022}.

Finally, the purpose of this literature is to study both passive and active approaches of doing causal inference, find ways to principally apply these methods given different problem setups, and examine accommodation for relaxing control studies for practical usage.


\begin{figure}[t]
        \centering
        \includegraphics[width=0.8\linewidth]{./figs/ci_causal_graphs.pdf}
        \caption{Examples of passive and active causal inference methods}
        \label{fig:ci_causal_graph}
\end{figure}



